Less is More: Summary of Long Instructions is Better for Program Synthesis

Despite the success of large pre-trained language models (LMs) such as Codex, they show below-par performance on the larger and more complicated programming related questions. We show that LMs benefit from the summarized version of complicated questions. Our findings show that superfluous information often present in problem description such as human characters, background stories, and names (which are included to help humans in understanding a task) does not help models in understanding a task. To this extent, we create a meta-dataset from the frequently used APPS dataset and the newly created CodeContests dataset for the program synthesis task. Our meta-dataset consists of human and synthesized summaries of the long and complicated programming questions. Experimental results on Codex show that our proposed approach outperforms baseline by 8.13% on the APPS dataset and 11.88% on the CodeContests dataset on average in terms of strict accuracy. Our analysis shows that summaries significantly improve performance for introductory (9.86%) and interview (11.48%) programming questions. However, it shows improvement by a small margin (~ 2%) for competitive programming questions, implying scope for future research in this direction.

==> EMNLP 2022/accuracy_results.tex <==
\begin{table*}[t!]
\centering
\small
\resizebox{0.95\linewidth}{!}{

\begin{tabular}{@{}lccc|ccc|ccc@{}}
% \begin{tabular}{@{}p{0.2\linewidth}p{0.2\linewidth}p{0.1\linewidth}p{0.1\linewidth}p{0.1\linewidth}@{}}
\toprule
\multirow{2}{*}{Difficulty} & \multicolumn{3}{c}{AP} & \multicolumn{3}{c}{EWPR} & \multicolumn{3}{c}{BWPR} \\ %& \multicolumn{1}{c}{Codex} \\
\cmidrule(lr){2-4}\cmidrule(lr){5-7}\cmidrule(lr){8-10}
~ & Baseline & Basic & Expert & Baseline & Basic & Expert & Baseline & Basic & Expert \\ %& Pass@1 \\ 
 \toprule
 Introductory & \textbf{57.76} & 56.06 & 53.72 & 57.97 & \textbf{58.67} & 57.98 & 57.64 & 57.22 & 54.84 \\ %& 4.14 \\
 Interview & 23.08 & 25.00 & \textbf{36.36} & 23.04 & 26.96 & \textbf{38.83} & 23.47 & 25.82 & \textbf{37.09} \\ %& 0.14 \\
 Competition & \textbf{19.22} & 18.06 & 18.32 & \textbf{20.31} & 18.85 & 18.78 & \textbf{19.43} & 18.40 & 18.66 \\ %& 0.02 \\
 \midrule
 Average & 27.65 & \textbf{29.28} & 28.61 & 28.96 & \textbf{33.15} & 32.45 & 28.36 & \textbf{31.47} & 30.52 \\
 \bottomrule
\end{tabular}
}
\caption{Results of baseline and proposed model in terms of Strict Accuracy (SAcc). All results are in \%. AP: All Problems, EWPR: Either Worst Problem Removal, BWPR: Both Worst Problem Removal (see explanation in section \ref{sec:exp-setup}).}
\label{tab:main-results}
\end{table*}

==> EMNLP 2022/agg_results.tex <==
\begin{table*}[t!]
\centering
\small
\resizebox{0.95\linewidth}{!}{

\begin{tabular}{@{}l|l|l|l|l|l@{}}
% \begin{tabular}{@{}p{0.2\linewidth}p{0.2\linewidth}p{0.1\linewidth}p{0.1\linewidth}p{0.1\linewidth}@{}}
\toprule
Experiment & Original Len & Summary Len & Orig Code Len & Summary Code Len & Code Solution Len\\
 \toprule
Summary & 1147 & 937 & 339 & 349 & 671 \\
 \midrule
Expert &  1147 & 869 & 339 & 343 & 671 \\
  \midrule
GPT & 1386 & 1011 & 437 & 392 & 748 \\
  \midrule
StudioAI21 & 1646 & 1114 & 602 & 473 & 721 \\
 \bottomrule
\end{tabular}
}
\caption{The average length of the original/summarized prompt and generated code. The average length of the code solutions is the average len of the solutions provided by the creators of the APPS dataset. A problem could have one or multiple solutions. The length is reported in characters.}
\label{tab:aggregate-results}
\end{table*}

==> EMNLP 2022/all_num_probs.tex <==
% \begin{table}[h]
% \centering
% \small
% \resizebox{0.85\linewidth}{!}{
% \begin{tabular}{@{}llll@{}}
% % \begin{tabular}{@{}p{0.2\linewidth}p{0.2\linewidth}p{0.1\linewidth}p{0.1\linewidth}p{0.1\linewidth}@{}}
% % \centering
% \toprule
% Data Source & Difficulty & \# of Problems \\
%  \toprule
%  \multirow{4}{*}{Human}
%  & Introductory & 161 \\
%  & Interview & 132 \\
%  & Competition & 121 \\
%  \midrule
%  & Total & 414 \\
%  \midrule
%  \multirow{4}{*}{Studio21}
%  & Introductory & 1514 \\
%  & Interview & 4531 \\
%  & Competition & 1275 \\
%  \midrule
%  & Total & 7320 \\
%  \midrule
%  \multirow{3}{*}{GPT-3}
%  & Interview & 250 \\
%  & Competition & 250 \\
%  \midrule
%  & Total & 500 \\ 
%  \bottomrule
% \end{tabular}
% }
% \caption{Statistics of the proposed meta-dataset.}
% \label{table:AllProblemNums}
% \end{table}

\begin{table}[h]
    \centering 
    \setlength\tabcolsep{4.0pt}
    \footnotesize
    
\resizebox{0.85\linewidth}{!}{
\begin{tabular}{ccc}
\toprule
\textbf{Data Source} & \textbf{Difficulty} & \textbf{\# of Problems} \\
 \midrule
 \multirow{4}{*}{Human}
 & Introductory & 145 \\
 & Interview & 123 \\
 & Competition & 105 \\
 & CodeContests & 80 \\
 \midrule
 & Total & 453 \\
 \midrule
 \multirow{4}{*}{Studio21}
 & Introductory & 1588 \\
 & Interview & 4551 \\
 & Competition & 1286 \\
 & CodeContests & 80 \\
 \midrule
 & Total & 7505 \\
 \midrule
 \multirow{3}{*}{GPT-3}
 & Introductory & 194 \\
 & Interview & 267 \\
 & Competition & 244 \\
 & CodeContests & 80 \\
 \midrule
 & Total & 785 \\ 
 \midrule
 \multirow{4}{*}{PEGASUS}
 & Introductory & 145 \\
 & Interview & 123 \\
 & Competition & 105 \\
 \midrule
 & Total & 373 \\
 \bottomrule
\end{tabular}
}
\caption{Statistics of the proposed meta-dataset.}
\label{table:AllProblemNums}
\end{table}

==> EMNLP 2022/compare_models.tex <==
\begin{table*}[t!]
\centering
\small
\resizebox{0.95\linewidth}{!}{

\begin{tabular}{@{}lcccc|cccc@{}}
\toprule
\multirow{2}{*}{Difficulty} & \multicolumn{4}{c}{AP} & \multicolumn{4}{c}{EWPR} \\ \\
\cmidrule(lr){2-5}\cmidrule(lr){6-9}\cmidrule(lr){10-13}
~ & Baseline & Basic & Expert & Baseline & Basic & Expert & Baseline & Basic & Expert \\ %& Pass@1 \\ 
 \toprule 
 Introductory & 42.96 & \textbf{50.00} & \textbf{50.00} &  44.20 & 51.45 & \textbf{51.82} & 43.23 & \textbf{50.35} & \textbf{50.35} \\ 
 Interview & 37.70 & 41.80 & \textbf{44.26} & 36.52 & 45.54 & \textbf{46.96} & 37.70 & 41.80 & \textbf{44.26} \\
 Competition & 4.76 & \textbf{5.71} & \textbf{5.71} & 4.00 & \textbf{6.00} & \textbf{6.00} & 4.76 & \textbf{5.71} & \textbf{5.71} \\
%  \midrule
%  Average & 28.47 & 32.50 & \textbf{33.32} & 28.24 & 34.00 & \textbf{34.93} & 28.56 & 32.62 & \textbf{33.44} \\
 \midrule
 Weighted Average & 30.35 & 34.69 & \textbf{35.50} & 30.31 & 36.65 & \textbf{37.22} & 30.43 & 34.78 & \textbf{35.59} \\
 \bottomrule
\end{tabular}
}
\caption{Results of baseline and proposed model in terms of Strict Accuracy (SAcc). All results are in \%. AP: All Problems, EWPR: Either Worst Problem Removal, BWPR: Both Worst Problem Removal (see explanation in section \ref{sec:exp-setup}).}
\label{tab:compare-resuls}
\end{table*}

==> EMNLP 2022/improvement_results.tex <==
\begin{table*}[t!]
\centering
\small
\resizebox{0.95\linewidth}{!}{
\begin{tabular}{lllll}
\hline
\multicolumn{1}{c}{Experiment} & Difficulty   & All Problems                        & Same/Better (one)                  & Same/Better (both) \\ \cline{3-5} 
\multicolumn{2}{l}{}                          & \multicolumn{1}{l|}{Improvement}    & \multicolumn{1}{l|}{Improvement}   & Improvement        \\ \hline
\multirow{3}{*}{Summary}       & Introductory & \multicolumn{1}{l|}{-0.62}          & \multicolumn{1}{l|}{2.72}          & \textbf{4.17}      \\
                               & Interview    & \multicolumn{1}{l|}{2.62}           & \multicolumn{1}{l|}{\textbf{6.02}} & 3.36               \\
                               & Competition  & \multicolumn{1}{l|}{2.48}           & \multicolumn{1}{l|}{2.71}          & \textbf{2.72}      \\ \hline
\multirow{3}{*}{Expert}        & Introductory & \multicolumn{1}{l|}{1.86}           & \multicolumn{1}{l|}{6.99}          & \textbf{7.64}      \\
                               & Interview    & \multicolumn{1}{l|}{2.61}           & \multicolumn{1}{l|}{\textbf{7.58}} & 3.38               \\
                               & Competition  & \multicolumn{1}{l|}{\textbf{-0.82}} & \multicolumn{1}{l|}{-0.89}         & -0.91             
\end{tabular}
}
\caption{This is the improvement for each experiment on each difficulty. This result of subtracting the Proposed column by the baseline column from \ref{tab:main-results}}
\label{tab:improvement-results}
\end{table*}

==> EMNLP 2022/main_results.tex <==
% \begin{table*}[t!]
% \centering
% \small
% \resizebox{0.95\linewidth}{!}{

% \begin{tabular}{@{}lccc|ccc|ccc@{}}
% % \begin{tabular}{@{}p{0.2\linewidth}p{0.2\linewidth}p{0.1\linewidth}p{0.1\linewidth}p{0.1\linewidth}@{}}
% \toprule
% \multirow{2}{*}{Difficulty} & \multicolumn{3}{c}{AP} & \multicolumn{3}{c}{EWPR} & \multicolumn{3}{c}{BWPR} \\ %& \multicolumn{1}{c}{Codex} \\
% \cmidrule(lr){2-4}\cmidrule(lr){5-7}\cmidrule(lr){8-10}
% ~ & Baseline & Basic & Expert & Baseline & Basic & Expert & Baseline & Basic & Expert \\ %& Pass@1 \\ 
%  \toprule
%  Introductory & \textbf{44.10} & 43.48 & 41.61 & 44.90 & \textbf{47.62} & 46.53 & 43.71 & \textbf{46.36} & 44.37 \\ %& 4.14 \\
%  Interview & 36.36 & 39.39 & \textbf{40.91} & 39.29 & 46.43 & \textbf{47.37} & 38.84 & 42.98 & \textbf{43.80}\\ %& 0.14 \\
%  Competition & 2.48 & \textbf{4.96} & 3.31 & 2.70 & \textbf{5.41} & 3.45 & 2.54 & \textbf{5.08} & 3.39 \\ %& 0.02 \\
%  \midrule
%  Average & 27.65 & \textbf{29.28} & 28.61 & 28.96 & \textbf{33.15} & 32.45 & 28.36 & \textbf{31.47} & 30.52 \\
%  \bottomrule
% \end{tabular}
% }
% \caption{Results of baseline and proposed model in terms of Strict Accuracy (SAcc). All results are in \%. AP: All Problems, EWPR: Either Worst Problem Removal, BWPR: Both Worst Problem Removal (see explanation in section \ref{sec:exp-setup}).}
% \label{tab:main-results}
% \end{table*}

\begin{table*}[t!]
    \centering 
    \setlength\tabcolsep{4.0pt}
    \footnotesize
\resizebox{0.95\linewidth}{!}{

\begin{tabular}{cccc|ccc|ccc}
% \begin{tabular}{@{}p{0.2\linewidth}p{0.2\linewidth}p{0.1\linewidth}p{0.1\linewidth}p{0.1\linewidth}@{}}
\toprule
\multirow{2}{*}{Difficulty} & \multicolumn{3}{c}{AP} & \multicolumn{3}{c}{EWPR} & \multicolumn{3}{c}{BWPR} \\ %& \multicolumn{1}{c}{Codex} \\
\cmidrule(lr){2-4}\cmidrule(lr){5-7}\cmidrule(lr){8-10}
~ & Baseline & Basic & Expert & Baseline & Basic & Expert & Baseline & Basic & Expert \\ %& Pass@1 \\ 
 \midrule 
 Introductory & 42.96 & \textbf{50.00} & \textbf{50.00} &  44.20 & 51.45 & \textbf{51.82} & 43.23 & \textbf{50.35} & \textbf{50.35} \\ 
 Interview & 37.70 & 41.80 & \textbf{44.26} & 36.52 & 45.54 & \textbf{46.96} & 37.70 & 41.80 & \textbf{44.26} \\
 Competition & 4.76 & \textbf{5.71} & \textbf{5.71} & 4.00 & \textbf{6.00} & \textbf{6.00} & 4.76 & \textbf{5.71} & \textbf{5.71} \\
%  \midrule
%  Average & 28.47 & 32.50 & \textbf{33.32} & 28.24 & 34.00 & \textbf{34.93} & 28.56 & 32.62 & \textbf{33.44} \\
 \midrule
 Weighted Average & 30.47 & 34.83 & \textbf{35.64} & 30.31 & 36.65 & \textbf{37.22} & 30.43 & 34.78 & \textbf{35.59} \\
 \midrule
  CodeContests & 12.50 & 23.75 & \textbf{25.00} & 13.33 & 25.33 & \textbf{26.66} & 12.82 & 24.36 & \textbf{25.64} \\
 \bottomrule
\end{tabular}
}
\caption{Results of baseline and proposed model in terms of Strict Accuracy (SAcc). The first block is from the APPS dataset. The last block is from the CodeContests dataset. AP: All Problems, EWPR: Either Worst Problem Removal, BWPR: Both Worst Problem Removal (see explanation in section \ref{sec:exp-setup}). All results are in \%. Weighted Average is not shown for CodeContests because similar difficulties were not provided (see explanation in \ref{sec:human-results}).}
\label{tab:main-results}
\end{table*}


% \begin{table*}[t!]
% \centering
% \small
% \resizebox{0.95\linewidth}{!}{

% \begin{tabular}{@{}lccc|ccc|ccc@{}}
% % \begin{tabular}{@{}p{0.2\linewidth}p{0.2\linewidth}p{0.1\linewidth}p{0.1\linewidth}p{0.1\linewidth}@{}}
% \toprule
% \multirow{2}{*}{Difficulty} & \multicolumn{3}{c}{AP} & \multicolumn{3}{c}{EWPR} & \multicolumn{3}{c}{BWPR} \\ %& \multicolumn{1}{c}{Codex} \\
% \cmidrule(lr){2-4}\cmidrule(lr){5-7}\cmidrule(lr){8-10}
% ~ & Baseline & Basic & Expert & Baseline & Basic & Expert & Baseline & Basic & Expert \\ %& Pass@1 \\ 
%  \toprule 
%  Introductory & 331 & \textbf{454} & 405 & 331 & \textbf{462} & 431 & 331 & \textbf{456} & 407 \\
%  Interview & 5 & 4 & \textbf{10} & 1 & 12 & \textbf{15} & 5 & 4 &\textbf{10} \\
%  Competition & -148 & \textbf{-39} & -71 & -158 & \textbf{-16} & -27 & -148 & \textbf{-39} & -71 \\ 
%  \midrule
%  Average & 62.66 & \textbf{139.66} & 114.66 & 58 & \textbf{152.66} & 139.66 & 62.66 & \textbf{140.33} & 115.33 \\
%  \bottomrule
% \end{tabular}
% }
% \caption{Results of baseline and proposed model in terms of test case score. All results are in \%. AP: All Problems, EWPR: Either Worst Problem Removal, BWPR: Both Worst Problem Removal (see explanation in section \ref{sec:exp-setup}).}
% \label{tab:main-score-results}
% \end{table*}

\begin{table}[t!]
\centering 
\setlength\tabcolsep{4.0pt}
\footnotesize
\resizebox{\linewidth}{!}{
\begin{tabular}{ccc|cc}
% \begin{tabular}{@{}p{0.2\linewidth}p{0.2\linewidth}p{0.1\linewidth}p{0.1\linewidth}p{0.1\linewidth}@{}}
\toprule
\multirow{2}{*}{Difficulty} & \multicolumn{2}{c}{AP} & \multicolumn{2}{c}{EWPR} \\
\cmidrule(lr){2-3}\cmidrule(lr){4-5}
~ & Baseline & Proposed & Baseline & Proposed \\ 
 \midrule
 Introductory & 42.96 & \textbf{52.82} & 44.53 & \textbf{54.74} \\
 Interview & 37.70 & \textbf{49.18} & 38.66 & \textbf{50.42} \\
 Competition & 4.76 & \textbf{6.67} & 4.81 & \textbf{6.73} \\
%  \midrule
%  Average & 28.47 & \textbf{36.22} & 29.33 & \textbf{37.30} \\
 \midrule
 Weighted Average & 30.47 & \textbf{38.48} & 31.11 & \textbf{39.44} \\
 \bottomrule
\end{tabular}
}
\caption{Results when taking the best summary for each problem. The EWPR baseline is different from Table \ref{tab:main-results} because a different set of problems have been removed.}
\label{tab:take-best}
\end{table}



==> EMNLP 2022/num_probs.tex <==
\begin{table}[t!]
\centering
\small
\resizebox{0.95\linewidth}{!}{

\begin{tabular}{@{}lll|l|l@{}}
% \begin{tabular}{@{}p{0.2\linewidth}p{0.2\linewidth}p{0.1\linewidth}p{0.1\linewidth}p{0.1\linewidth}@{}}
\toprule
Summary & Difficulty & AP & EWPR & BWPR\\
 \toprule
 \multirow{3}{*}{Basic}
 & Introductory & 145 & 141 & 144 \\
 & Interview & 123 & 113 & 123 \\
 & Competition & 105 & 100 & 105 \\
 \midrule
 \multirow{3}{*}{Expert}
 & Introductory & 145 & 140 & 144 \\
 & Interview & 123 & 116 & 123 \\
 & Competition & 105 & 100 & 105 \\
 \midrule
  \multirow{3}{*}{StudioAI21}
 & Introductory & 215 & 187 & - \\
 & Interview & 627 & 558 & - \\
 & Competition & 659 & 578 & - \\
 \midrule
  \multirow{3}{*}{GPT3}
 & Introductory & 194 & 180 & - \\
 & Interview & 266 & 242 & - \\
 & Competition & 244 & 220 & - \\
 \bottomrule
\end{tabular}
}
\caption{These are the numbers of problems in each split of the dataset. For GPT and Studio21 we did not look at problems that were worse or same for both experiments because there was insignificant overlap between the two experiments.}
\label{tab:number-of-probs}
\end{table}

==> EMNLP 2022/old_main_results.tex <==
\begin{table*}[t!]
\centering
\small
\resizebox{0.95\linewidth}{!}{

\begin{tabular}{@{}llcc|cc|ccc@{}}
% \begin{tabular}{@{}p{0.2\linewidth}p{0.2\linewidth}p{0.1\linewidth}p{0.1\linewidth}p{0.1\linewidth}@{}}
\toprule
\multirow{2}{*}{Experiment} & \multirow{2}{*}{Difficulty} & \multicolumn{2}{c}{All Problems} & \multicolumn{2}{c}{EWPR} & \multicolumn{2}{c}{BWPR} \\ %& \multicolumn{1}{c}{Codex} \\
\cmidrule(lr){3-4}\cmidrule(lr){5-6}\cmidrule(lr){7-8}
~& ~ & Baseline & Proposed & Baseline & Proposed & Baseline & Proposed \\ %& Pass@1 \\ 
 \toprule
 \multirow{3}{*}{Basic Summary}
 & Introductory & \textbf{44.10} & 43.48 & 44.90 & \textbf{47.62} & 44.44 & \textbf{48.61} \\ %& 4.14 \\
 & Interview & 36.36 & \textbf{39.39} & 39.29 & \textbf{46.43} & 37.01 & \textbf{40.94} \\ %& 0.14 \\
 & Competition & 2.48 & \textbf{4.96} & 2.70 & \textbf{5.41} & 2.73 & \textbf{5.45} \\ %& 0.02 \\
 \midrule
 \multirow{3}{*}{Expert Summary}
 & Introductory & 42.86 & \textbf{44.72} & 43.36 & \textbf{50.35} & 42.36 & \textbf{50.00} \\ %& 4.14 \\
 & Interview & 37.88 & \textbf{40.91} & 39.64 & \textbf{48.65} & 38.58 & \textbf{42.52} \\ %& 0.14 \\
 & Competition & \textbf{4.13} & 3.31 & \textbf{4.46} & 3.57 & \textbf{4.55} & 3.64 \\ %& 0.02 \\
 \bottomrule
\end{tabular}
}
\caption{Results of baseline and proposed model in terms of Strict Accuracy (SAcc). All results are in \%.}
\label{tab:old-main-results}
\end{table*}

==> EMNLP 2022/old_num_probs.tex <==
\begin{table*}[t!]
\centering
\small
\resizebox{0.95\linewidth}{!}{

\begin{tabular}{@{}lll|l|l@{}}
% \begin{tabular}{@{}p{0.2\linewidth}p{0.2\linewidth}p{0.1\linewidth}p{0.1\linewidth}p{0.1\linewidth}@{}}
\toprule
Experiment & Difficulty & All Problems & Same/Better (one) & Same/Better (both)\\
 \toprule
 \multirow{3}{*}{Summary}
 & Introductory & 162 & 147 & 144 \\
 & Interview & 152 & 133 & 148 \\
 & Competition & 121 & 111 & 110 \\
 \midrule
 \multirow{3}{*}{Expert}
 & Introductory & 162 & 143 & 144 \\
 & Interview & 152 & 132 & 148 \\
 & Competition & 121 & 112 & 110 \\
  \midrule
 \multirow{3}{*}{GPT}
 & Introductory & - & - & - \\
 & Interview & 250 & 211 & - \\
 & Competition & 250 & 223 & -\\
  \midrule
 \multirow{3}{*}{Studio21}
 & Introductory & 228 & 193 & - \\
 & Interview & 374 & 322 & -\\
 & Competition & 398 & 338 & -\\
 \bottomrule
\end{tabular}
}
\caption{These are the numbers of problems in each split of the dataset. For GPT and Studio21 we did not look at problems that were worse or same for both experiments because there was insignificant overlap between the two experiments.}
\label{tab:old-number-of-probs}
\end{table*}

==> EMNLP 2022/old_syn_results.tex <==
\begin{table*}[t!]
\centering
\small
\resizebox{0.95\linewidth}{!}{

\begin{tabular}{@{}llcc|cc|c@{}}
% \begin{tabular}{@{}p{0.2\linewidth}p{0.2\linewidth}p{0.1\linewidth}p{0.1\linewidth}p{0.1\linewidth}@{}}
\toprule
\multirow{2}{*}{Experiment} & \multirow{2}{*}{Difficulty} & \multicolumn{2}{c}{All Problems} & \multicolumn{2}{c}{Same/Better (one)} & \multicolumn{1}{c}{Codex} \\
\cmidrule(lr){3-4}\cmidrule(lr){5-6}
~& ~ & Baseline & Proposed & Baseline & Proposed & Pass@1 \\ 
 \toprule
 \multirow{2}{*}{GPT}
 & Interview & \textbf{5.2} & 4.8 & 4.74 & \textbf{5.69} & 0.14\\
 & Competition & 0.40 & 0.80 & \textbf{0.45} & \textbf{0.90} & 0.02\\
 \midrule
 \multirow{3}{*}{Studio21}
 & Introductory & 53.95 & 47.37 & \textbf{56.48} & \textbf{55.96} & 4.14\\
 & Interview & \textbf{14.44} & 10.70 & 11.18 & \textbf{12.42} & 0.14\\
 & Competition & \textbf{1.76} & 1.51 & 1.48 & \textbf{1.78} & 0.02\\
 \bottomrule
\end{tabular}
}
\caption{The strict accuracy of our experiments on synthetically generated summaries. 500 summaries generated by GPT were tested and 1000 summaries generated by StudioAI21 were tested. Because there was little overlap between the different experiments we did not calculate results for Same/Better(both) as in table \ref{tab:main-results}}
\label{tab:synthetic-results}
\end{table*}

==> EMNLP 2022/pegasus_results.tex <==
\begin{table}[t!]
\centering 
\setlength\tabcolsep{4.0pt}
\footnotesize
\resizebox{\linewidth}{!}{
\begin{tabular}{ccc|cc}
% \begin{tabular}{@{}p{0.2\linewidth}p{0.2\linewidth}p{0.1\linewidth}p{0.1\linewidth}p{0.1\linewidth}@{}}
\toprule
\multirow{2}{*}{Difficulty} & \multicolumn{2}{c}{AP} & \multicolumn{2}{c}{EWPR} \\
\cmidrule(lr){2-3}\cmidrule(lr){4-5}
~ & Baseline & PEGASUS & Baseline & PEGASUS \\ 
 \midrule
 Introductory & \textbf{42.96} & 34.48 & \textbf{44.26} & 40.98 \\
 Interview & \textbf{37.70} & 10.57 & 14.29 & \textbf{21.56}   \\
 Competition & \textbf{4.76} & 0.00 & \textbf{2.76} & 0.00 \\
%  \midrule
%  Average & 28.47 & \textbf{36.22} & 29.33 & \textbf{37.30} \\
 \midrule
 Weighted Average & 30.47 & \textbf{16.88} & \textbf{25.50} & 24.73 \\
 \bottomrule
\end{tabular}
}
\caption{Results of the Pegasus on the APPS dataset. Although the EWPR results for PEGASUS are better a significant portion of the problems performed worse. An exact count for the problems is found in \ref{tab:pegasus-num-prob}}}
\label{tab:pegasus-results}
\end{table}

\begin{table}[t!]
\centering
\small
\resizebox{0.95\linewidth}{!}{

\begin{tabular}{@{}lll|l@{}}
% \begin{tabular}{@{}p{0.2\linewidth}p{0.2\linewidth}p{0.1\linewidth}p{0.1\linewidth}p{0.1\linewidth}@{}}
\toprule
Model & Difficulty & AP & EWPR \\
 \toprule
 \multirow{4}{*}{Pegasus}
 & Introductory & 145 & 122 \\
 & Interview & 123 & 56 \\
 & Competition & 105 & 73 \\
 \midrule
%  \multirow{1}{*}{Pegasus}
 & Total & 373 & 251 \\
 \bottomrule
\end{tabular}
}
\caption{\kirby{These are the numbers of problems in each split. The number of problems dips significantly for the EWPR experiment.}}
\label{tab:pegasus-num-prob}
\end{table}


==> EMNLP 2022/short-synthetic-results.tex <==
\begin{table}[t!]
\centering
\small
\resizebox{\linewidth}{!}{

\begin{tabular}{@{}llcc|cc@{}}
% \begin{tabular}{@{}p{0.2\linewidth}p{0.2\linewidth}p{0.1\linewidth}p{0.1\linewidth}p{0.1\linewidth}@{}}
\toprule
\multirow{2}{*}{Model} & \multirow{2}{*}{Difficulty} & \multicolumn{2}{c}{AP} & \multicolumn{2}{c}{EWPR} \\
\cmidrule(lr){3-4}\cmidrule(lr){5-6}
~& ~ & Baseline & Proposed & Baseline & Proposed \\ 
 \toprule
 \multirow{2}{*}{GPT-3}
 & Introductory & \textbf{41.97} & 38.86 & 41.11 & \textbf{41.67} \\
 & Interview & 25.27 & \textbf{27.47} & 24.86 & \textbf{28.25} \\
 & Competition & 4.80 & \textbf{6.40} & 4.88 & \textbf{6.50} \\
 \midrule
 & Weighted Average & \textbf{26.60} & \textbf{26.60} & 25.83 & \textbf{27.71} \\
 \midrule
 \multirow{3}{*}{Studio21}
 & Introductory & \textbf{39.91} & 31.92 & \textbf{39.25} & 36.56 \\
 & Interview & \textbf{15.97} & 14.50 & 13.23 & \textbf{15.47} \\
 & Competition & \textbf{2.57} & \textbf{2.57} & \textbf{2.71} & \textbf{2.71} \\
 \midrule
 & Weighted Average & \textbf{16.90} & 14.50 & 15.10 & \textbf{15.64} \\
 \bottomrule
\end{tabular}
}
\caption{Results when taking the top 500 GPT problems and top 1000 Studio problems}
\label{tab:condensed-synthetic-results}
\end{table}

==> EMNLP 2022/synthetic_results.tex <==
\begin{table*}[ht]
\centering 
\setlength\tabcolsep{4.0pt}
\footnotesize
\resizebox{0.75\linewidth}{!}{

\begin{tabular}{cccc|cc}
% \begin{tabular}{@{}p{0.2\linewidth}p{0.2\linewidth}p{0.1\linewidth}p{0.1\linewidth}p{0.1\linewidth}@{}}
\toprule
\multirow{2}{*}{Model} & \multirow{2}{*}{Difficulty} & \multicolumn{2}{c}{AP} & \multicolumn{2}{c}{EWPR} \\
\cmidrule(lr){3-4}\cmidrule(lr){5-6}
~& ~ & Baseline & Proposed & Baseline & Proposed \\ 
 \midrule
 \multirow{2}{*}{GPT-3}
 & Introductory & \textbf{41.75} & 38.66 & 41.11 & \textbf{41.67} \\
 & Interview & \textbf{20.30} & 18.80 & 18.18 & \textbf{20.66} \\
 & Competition & 2.87 & \textbf{3.28} & 2.73 & \textbf{3.64} \\
 \midrule
 & Weighted Average & \textbf{20.17} & 18.89 & 19.14 & \textbf{20.55} \\
 \midrule
 \multirow{3}{*}{Studio21}
 & Introductory & \textbf{39.53} & 31.63 & \textbf{39.04} & 36.36 \\
 & Interview & \textbf{12.28} & 11.00 & 10.57 & \textbf{12.37} \\
 & Competition & \textbf{1.67} & 1.21 & \textbf{1.38} & \textbf{1.38}\\
 \midrule
 & Weighted Average & \textbf{11.53} & 9.66 & 10.61 & \textbf{10.98} \\
 \midrule
 \multirow{3}{*}{PEGASUS}
 & Introductory & \textbf{42.96} & 34.48 & \textbf{44.26} & 40.98 \\
 & Interview & \textbf{37.70} & 10.57 & 14.29 & \textbf{21.56}   \\
 & Competition & \textbf{4.76} & 0.00 & \textbf{2.76} & 0.00 \\
 \midrule
 & Weighted Average & \textbf{30.47} & 16.88 & \textbf{25.50} & 24.73 \\
 \bottomrule
\end{tabular}
}
\caption{Results of baseline and proposed approach (All results are in \%). Summaries generated by GPT-3, Studio21, and PEGASUS used for inference from APPS.}
% 704 summaries generated by GPT-3, 1501 summaries generated by Studio21, and 453 summaries generated by PEGASUS used for inference from APPS.
\label{tab:synthetic-results}
\end{table*}

\begin{table}[ht]
\centering 
\setlength\tabcolsep{4.0pt}
\footnotesize
\resizebox{\linewidth}{!}{

\begin{tabular}{ccc|cc}
% \begin{tabular}{@{}p{0.2\linewidth}p{0.2\linewidth}p{0.1\linewidth}p{0.1\linewidth}p{0.1\linewidth}@{}}
\toprule
\multirow{2}{*}{Model} & \multicolumn{2}{c}{AP} & \multicolumn{2}{c}{EWPR} \\
\cmidrule(lr){2-3}\cmidrule(lr){4-5}
~ & Baseline & Proposed & Baseline & Proposed \\ 
 \midrule
 \multirow{1}{*}{GPT-3}
 & \textbf{12.50} & 10.0 & \textbf{18.75} & \textbf{18.75} \\
 \midrule
 \multirow{1}{*}{Studio21}
 & \textbf{12.50} & 8.75 & \textbf{22.5} & 20.0 \\
 \bottomrule
\end{tabular}
}
\caption{Results of baseline and proposed approach (All results are in \%). 80 summaries generated by GPT-3 and Studio21 used for inference from CodeContests.}
\label{tab:code-contests-synthetic-results}
\end{table}


==> accuracy_results.tex <==
\begin{table*}[t!]
\centering
\small
\resizebox{0.95\linewidth}{!}{

\begin{tabular}{@{}lccc|ccc|ccc@{}}
% \begin{tabular}{@{}p{0.2\linewidth}p{0.2\linewidth}p{0.1\linewidth}p{0.1\linewidth}p{0.1\linewidth}@{}}
\toprule
\multirow{2}{*}{Difficulty} & \multicolumn{3}{c}{AP} & \multicolumn{3}{c}{EWPR} & \multicolumn{3}{c}{BWPR} \\ %& \multicolumn{1}{c}{Codex} \\
\cmidrule(lr){2-4}\cmidrule(lr){5-7}\cmidrule(lr){8-10}
~ & Baseline & Basic & Expert & Baseline & Basic & Expert & Baseline & Basic & Expert \\ %& Pass@1 \\ 
 \toprule
 Introductory & \textbf{57.76} & 56.06 & 53.72 & 57.97 & \textbf{58.67} & 57.98 & 57.64 & 57.22 & 54.84 \\ %& 4.14 \\
 Interview & 23.08 & 25.00 & \textbf{36.36} & 23.04 & 26.96 & \textbf{38.83} & 23.47 & 25.82 & \textbf{37.09} \\ %& 0.14 \\
 Competition & \textbf{19.22} & 18.06 & 18.32 & \textbf{20.31} & 18.85 & 18.78 & \textbf{19.43} & 18.40 & 18.66 \\ %& 0.02 \\
 \midrule
 Average & 27.65 & \textbf{29.28} & 28.61 & 28.96 & \textbf{33.15} & 32.45 & 28.36 & \textbf{31.47} & 30.52 \\
 \bottomrule
\end{tabular}
}
\caption{Results of baseline and proposed model in terms of Strict Accuracy (SAcc). All results are in \%. AP: All Problems, EWPR: Either Worst Problem Removal, BWPR: Both Worst Problem Removal (see explanation in section \ref{sec:exp-setup}).}
\label{tab:main-results}
\end{table*}

==> compare_models.tex <==
\begin{table*}[t!]
\centering
\small
\resizebox{0.95\linewidth}{!}{

\begin{tabular}{@{}lcccc|cccc@{}}
\toprule
\multirow{2}{*}{Difficulty} & \multicolumn{4}{c}{AP} & \multicolumn{4}{c}{EWPR} \\ \\
\cmidrule(lr){2-5}\cmidrule(lr){6-9}\cmidrule(lr){10-13}
~ & Baseline & Basic & Expert & Baseline & Basic & Expert & Baseline & Basic & Expert \\ %& Pass@1 \\ 
 \toprule 
 Introductory & 42.96 & \textbf{50.00} & \textbf{50.00} &  44.20 & 51.45 & \textbf{51.82} & 43.23 & \textbf{50.35} & \textbf{50.35} \\ 
 Interview & 37.70 & 41.80 & \textbf{44.26} & 36.52 & 45.54 & \textbf{46.96} & 37.70 & 41.80 & \textbf{44.26} \\
 Competition & 4.76 & \textbf{5.71} & \textbf{5.71} & 4.00 & \textbf{6.00} & \textbf{6.00} & 4.76 & \textbf{5.71} & \textbf{5.71} \\
%  \midrule
%  Average & 28.47 & 32.50 & \textbf{33.32} & 28.24 & 34.00 & \textbf{34.93} & 28.56 & 32.62 & \textbf{33.44} \\
 \midrule
 Weighted Average & 30.35 & 34.69 & \textbf{35.50} & 30.31 & 36.65 & \textbf{37.22} & 30.43 & 34.78 & \textbf{35.59} \\
 \bottomrule
\end{tabular}
}
\caption{Results of baseline and proposed model in terms of Strict Accuracy (SAcc). All results are in \%. AP: All Problems, EWPR: Either Worst Problem Removal, BWPR: Both Worst Problem Removal (see explanation in section \ref{sec:exp-setup}).}
\label{tab:compare-resuls}
\end{table*}

==> improvement_results.tex <==
\begin{table*}[t!]
\centering
\small
\resizebox{0.95\linewidth}{!}{
\begin{tabular}{lllll}
\hline
\multicolumn{1}{c}{Experiment} & Difficulty   & All Problems                        & Same/Better (one)                  & Same/Better (both) \\ \cline{3-5} 
\multicolumn{2}{l}{}                          & \multicolumn{1}{l|}{Improvement}    & \multicolumn{1}{l|}{Improvement}   & Improvement        \\ \hline
\multirow{3}{*}{Summary}       & Introductory & \multicolumn{1}{l|}{-0.62}          & \multicolumn{1}{l|}{2.72}          & \textbf{4.17}      \\
                               & Interview    & \multicolumn{1}{l|}{2.62}           & \multicolumn{1}{l|}{\textbf{6.02}} & 3.36               \\
                               & Competition  & \multicolumn{1}{l|}{2.48}           & \multicolumn{1}{l|}{2.71}          & \textbf{2.72}      \\ \hline
\multirow{3}{*}{Expert}        & Introductory & \multicolumn{1}{l|}{1.86}           & \multicolumn{1}{l|}{6.99}          & \textbf{7.64}      \\
                               & Interview    & \multicolumn{1}{l|}{2.61}           & \multicolumn{1}{l|}{\textbf{7.58}} & 3.38               \\
                               & Competition  & \multicolumn{1}{l|}{\textbf{-0.82}} & \multicolumn{1}{l|}{-0.89}         & -0.91             
\end{tabular}
}
\caption{This is the improvement for each experiment on each difficulty. This result of subtracting the Proposed column by the baseline column from \ref{tab:main-results}}
\label{tab:improvement-results}
\end{table*}

==> old_main_results.tex <==
\begin{table*}[t!]
\centering
\small
\resizebox{0.95\linewidth}{!}{

\begin{tabular}{@{}llcc|cc|ccc@{}}
% \begin{tabular}{@{}p{0.2\linewidth}p{0.2\linewidth}p{0.1\linewidth}p{0.1\linewidth}p{0.1\linewidth}@{}}
\toprule
\multirow{2}{*}{Experiment} & \multirow{2}{*}{Difficulty} & \multicolumn{2}{c}{All Problems} & \multicolumn{2}{c}{EWPR} & \multicolumn{2}{c}{BWPR} \\ %& \multicolumn{1}{c}{Codex} \\
\cmidrule(lr){3-4}\cmidrule(lr){5-6}\cmidrule(lr){7-8}
~& ~ & Baseline & Proposed & Baseline & Proposed & Baseline & Proposed \\ %& Pass@1 \\ 
 \toprule
 \multirow{3}{*}{Basic Summary}
 & Introductory & \textbf{44.10} & 43.48 & 44.90 & \textbf{47.62} & 44.44 & \textbf{48.61} \\ %& 4.14 \\
 & Interview & 36.36 & \textbf{39.39} & 39.29 & \textbf{46.43} & 37.01 & \textbf{40.94} \\ %& 0.14 \\
 & Competition & 2.48 & \textbf{4.96} & 2.70 & \textbf{5.41} & 2.73 & \textbf{5.45} \\ %& 0.02 \\
 \midrule
 \multirow{3}{*}{Expert Summary}
 & Introductory & 42.86 & \textbf{44.72} & 43.36 & \textbf{50.35} & 42.36 & \textbf{50.00} \\ %& 4.14 \\
 & Interview & 37.88 & \textbf{40.91} & 39.64 & \textbf{48.65} & 38.58 & \textbf{42.52} \\ %& 0.14 \\
 & Competition & \textbf{4.13} & 3.31 & \textbf{4.46} & 3.57 & \textbf{4.55} & 3.64 \\ %& 0.02 \\
 \bottomrule
\end{tabular}
}
\caption{Results of baseline and proposed model in terms of Strict Accuracy (SAcc). All results are in \%.}
\label{tab:old-main-results}
\end{table*}

==> old_num_probs.tex <==
\begin{table*}[t!]
\centering
\small
\resizebox{0.95\linewidth}{!}{

\begin{tabular}{@{}lll|l|l@{}}
% \begin{tabular}{@{}p{0.2\linewidth}p{0.2\linewidth}p{0.1\linewidth}p{0.1\linewidth}p{0.1\linewidth}@{}}
\toprule
Experiment & Difficulty & All Problems & Same/Better (one) & Same/Better (both)\\
 \toprule
 \multirow{3}{*}{Summary}
 & Introductory & 162 & 147 & 144 \\
 & Interview & 152 & 133 & 148 \\
 & Competition & 121 & 111 & 110 \\
 \midrule
 \multirow{3}{*}{Expert}
 & Introductory & 162 & 143 & 144 \\
 & Interview & 152 & 132 & 148 \\
 & Competition & 121 & 112 & 110 \\
  \midrule
 \multirow{3}{*}{GPT}
 & Introductory & - & - & - \\
 & Interview & 250 & 211 & - \\
 & Competition & 250 & 223 & -\\
  \midrule
 \multirow{3}{*}{Studio21}
 & Introductory & 228 & 193 & - \\
 & Interview & 374 & 322 & -\\
 & Competition & 398 & 338 & -\\
 \bottomrule
\end{tabular}
}
\caption{These are the numbers of problems in each split of the dataset. For GPT and Studio21 we did not look at problems that were worse or same for both experiments because there was insignificant overlap between the two experiments.}
\label{tab:old-number-of-probs}
\end{table*}

==> old_syn_results.tex <==
\begin{table*}[t!]
\centering
\small
\resizebox{0.95\linewidth}{!}{

\begin{tabular}{@{}llcc|cc|c@{}}
% \begin{tabular}{@{}p{0.2\linewidth}p{0.2\linewidth}p{0.1\linewidth}p{0.1\linewidth}p{0.1\linewidth}@{}}
\toprule
\multirow{2}{*}{Experiment} & \multirow{2}{*}{Difficulty} & \multicolumn{2}{c}{All Problems} & \multicolumn{2}{c}{Same/Better (one)} & \multicolumn{1}{c}{Codex} \\
\cmidrule(lr){3-4}\cmidrule(lr){5-6}
~& ~ & Baseline & Proposed & Baseline & Proposed & Pass@1 \\ 
 \toprule
 \multirow{2}{*}{GPT}
 & Interview & \textbf{5.2} & 4.8 & 4.74 & \textbf{5.69} & 0.14\\
 & Competition & 0.40 & 0.80 & \textbf{0.45} & \textbf{0.90} & 0.02\\
 \midrule
 \multirow{3}{*}{Studio21}
 & Introductory & 53.95 & 47.37 & \textbf{56.48} & \textbf{55.96} & 4.14\\
 & Interview & \textbf{14.44} & 10.70 & 11.18 & \textbf{12.42} & 0.14\\
 & Competition & \textbf{1.76} & 1.51 & 1.48 & \textbf{1.78} & 0.02\\
 \bottomrule
\end{tabular}
}
\caption{The strict accuracy of our experiments on synthetically generated summaries. 500 summaries generated by GPT were tested and 1000 summaries generated by StudioAI21 were tested. Because there was little overlap between the different experiments we did not calculate results for Same/Better(both) as in table \ref{tab:main-results}}
\label{tab:synthetic-results}
\end{table*}

==> pegasus_results.tex <==
\begin{table}[t!]
\centering 
\setlength\tabcolsep{4.0pt}
\footnotesize
\resizebox{\linewidth}{!}{
\begin{tabular}{ccc|cc}
% \begin{tabular}{@{}p{0.2\linewidth}p{0.2\linewidth}p{0.1\linewidth}p{0.1\linewidth}p{0.1\linewidth}@{}}
\toprule
\multirow{2}{*}{Difficulty} & \multicolumn{2}{c}{AP} & \multicolumn{2}{c}{EWPR} \\
\cmidrule(lr){2-3}\cmidrule(lr){4-5}
~ & Baseline & PEGASUS & Baseline & PEGASUS \\ 
 \midrule
 Introductory & \textbf{42.96} & 34.48 & \textbf{44.26} & 40.98 \\
 Interview & \textbf{37.70} & 10.57 & 14.29 & \textbf{21.56}   \\
 Competition & \textbf{4.76} & 0.00 & \textbf{2.76} & 0.00 \\
%  \midrule
%  Average & 28.47 & \textbf{36.22} & 29.33 & \textbf{37.30} \\
 \midrule
 Weighted Average & 30.47 & \textbf{16.88} & \textbf{25.50} & 24.73 \\
 \bottomrule
\end{tabular}
}
\caption{Results of the Pegasus on the APPS dataset. Although the EWPR results for PEGASUS are better a significant portion of the problems performed worse. An exact count for the problems is found in \ref{tab:pegasus-num-prob}}}
\label{tab:pegasus-results}
\end{table}

\begin{table}[t!]
\centering
\small
\resizebox{0.95\linewidth}{!}{

\begin{tabular}{@{}lll|l@{}}
% \begin{tabular}{@{}p{0.2\linewidth}p{0.2\linewidth}p{0.1\linewidth}p{0.1\linewidth}p{0.1\linewidth}@{}}
\toprule
Model & Difficulty & AP & EWPR \\
 \toprule
 \multirow{4}{*}{Pegasus}
 & Introductory & 145 & 122 \\
 & Interview & 123 & 56 \\
 & Competition & 105 & 73 \\
 \midrule
%  \multirow{1}{*}{Pegasus}
 & Total & 373 & 251 \\
 \bottomrule
\end{tabular}
}
\caption{\kirby{These are the numbers of problems in each split. The number of problems dips significantly for the EWPR experiment.}}
\label{tab:pegasus-num-prob}
\end{table}

